GreenWhisk: Emission-Aware Computing for Serverless Platform

Serverless computing is an emerging cloud computing abstraction wherein the cloud platform transparently manages all resources, including explicitly provisioning resources and geographical load balancing when the demand for service spikes. Users provide code as functions, and the cloud platform runs these functions handling all aspects of function execution. While prior work has primarily focused on optimizing performance, this paper focuses on reducing the carbon footprint of these systems making variations in grid carbon intensity and intermittency from renewables transparent to the user. We introduce GreenWhisk, a carbon-aware serverless computing platform built upon Apache OpenWhisk, operating in two modes - grid-connected and grid-isolated - addressing intermittency challenges arising from renewables and the grid's carbon footprint. Moreover, we develop carbon-aware load balancing algorithms that leverage energy and carbon information to reduce the carbon footprint. Our evaluation results show that GreenWhisk can easily incorporate carbon-aware algorithms, thereby reducing the carbon footprint of functions without significantly impacting the performance of function execution. In doing so, our system design enables the integration of new carbon-aware strategies into a serverless computing platform.

==> weighted_pseudo_v1.tex <==
\begin{algorithm}
\caption{Carbon-aware Load Balancing}\label{alg:one}
\begin{algorithmic}
\Procedure{distance}{$server$, $function$}
  \State \Return $-\log(\ [\ 1 - (server - function) ]\ \%\ 1\ )$
\EndProcedure
\Procedure{weight\_grid\_isolated}{$i$, $available\_energy$}
  \State \Return $available\_energy_i / \sum_j available\_energy_j $
\EndProcedure
\Procedure{weight\_grid\_conn}{ $i$, $carbon\_intensity$ }
  \State \Return $- carbon\_intensity_i / \sum_j carbon\_intensity_j $
\EndProcedure
\Procedure{sort\_servers}{$servers$, $function$, $metric$}
    \State $s\_list \gets [ ] $
    \For{$s \in servers$}
        \State $d \gets  distance(s, function)$
        \If {$grid\_connected$}
            \State $w \gets d\ /\ weight\_grid\_conn(s, metric)$
        \Else
            % \If {grid\_isolated}
            \State $w \gets d\ /\ weight\_grid\_isolated(s, metric)$
            % \EndIf
        \EndIf
        \State $s\_list.append((s, w))$
    \EndFor
    \State $s\_list \gets s\_list.sort(key=operator.itemgetter(1)) 
    $\Comment{sorts tuple by weight}
    \State \Return $s\_list$
\EndProcedure
\Procedure{select\_server}{$servers$, $function$, $metric$}
    \State $c \gets None$
    \For{$s \in sort\_servers(servers)$}
        \If {$s.memory < mem\_limit$}
            \State $c \gets s$
            \State \textbf{break}
        \EndIf
    \EndFor
    \If{$c$ \textbf{is} $None$}
        \State $retry\_queue.add(function)$
    \Else
        \State $s.invoke(function)$
    \EndIf
\EndProcedure
% \textcolor{red}{Add the forwarding policy}
\end{algorithmic}
% \begin{algorithmic}
% \State $height(A, B) \gets -log(\ [\ 1 - (A - B) ]\ \%\ 1\ )$
% \State $weight(A) \gets energy(A)\ /\ sum(energy)$
% \Procedure{sort\_servers}{$servers$, $function$}
%     \For{$s \in servers$}
%         \State $d \gets  distance(s, function)$
%         \If {$grid\_connected$}
%             \State $w \gets height\ /\ weight(node)$
%         \Else
%             \If {grid\_isolated}
%             \State $w \gets height\ /\ weight(node)$
%         \EndIf
%     \EndFor
% \State $Nodes \gets sorted(Nodes, Metric)$
% \EndProcedure
% \end{algorithmic}
\end{algorithm}

